Wi-Closure: Reliable and Efficient Search of Inter-robot Loop Closures Using Wireless Sensing

In this paper we propose a novel algorithm, Wi-Closure, to improve computational efficiency and robustness of loop closure detection in multi-robot SLAM. Our approach decreases the computational overhead of classical approaches by pruning the search space of potential loop closures, prior to evaluation by a typical multi-robot SLAM pipeline. Wi-Closure achieves this by identifying candidates that are spatially close to each other by using sensing over the wireless communication signal between robots, even when they are operating in non-line-of-sight or in remote areas of the environment from one another. We demonstrate the validity of our approach in simulation and hardware experiments. Our results show that using Wi-closure greatly reduces computation time, by 54% in simulation and by 77% in hardware compared, with a multi-robot SLAM baseline. Importantly, this is achieved without sacrificing accuracy. Using Wi-Closure reduces absolute trajectory estimation error by 99% in simulation and 89.2% in hardware experiments. This improvement is due in part to Wi-Closure's ability to avoid catastrophic optimization failure that typically occurs with classical approaches in challenging repetitive environments.

==> Chapters/OLD/1_Introduction.tex <==
\section{Introduction}
Loop closure detection has been widely studied as a fundamental aspect of Simultaneous localization and mapping (SLAM) \cite{loop-closure-slam}. The location estimate of the robot drifts over time due to noise in the on-board odometer; therefore, loop closure detection is essential as it corrects for this drift by recognizing previously visited places. Without such corrections, the world as perceived by the robot may diverge too much from reality, which could leave a robot unable to efficiently act. %Consequently, loop closure detection is a vital tool to obtain consistent map and location estimates such that these accumulating errors do not deter the robot from completing its task, especially in GPS-denied environments.
Similarly, if multiple robots intend to collaborate, they require a shared situational awareness that is sufficiently consistent with reality, as obtained by multi-robot SLAM. The key to obtaining this shared understanding is inter-robot loop closures. Where regular loop closures constrain the positions of one robot, inter-robot loop closures define a spatial relation between pairs of robots. These enable the robots to merge local sensor data into a shared model of the world and obtain their relative locations. There are generally two methods for finding inter-robot loop closures: robots directly observe and identify each other, or robots recognize that they have visited the same place. The first option requires robots to rendezvous with direct-line view, which is a non-trivial task if they do not know where they are positioned relative to each other. Therefore, many works focus on how to make the second option viable. %, which include various steps including 1) locally extracting salient features from vision or LiDAR data, 2) sharing of the features with other robots, and 3) matching similar features to recognize previously visited places. 


%Particularly, inter-robot loop closure has been paid additional attention given the benefits of deploying multiple robots in the field to explore, map, and share the environment information more efficiently. This process usually involves multiple stages of processing between robot including: locally extract local features from vision or lidar data, share the extracted features with others, iterate over all features from different different robot to find the common features that have been visited before.
% Map creation is an already well investigated topic in the Robotics community in terms of single robot SLAM. We investigate the problem of optimizing map merging within a multi-robot system using SLAM and checking for robustness in a scenario where communication may be limited such that continuous communication is unavailable. \\


%If a reliable estimate of the relative positions of the robots were available, this would considerably alleviate the problem as we could connect the odometry backbones of the robots and assess whether a potential inter-robot loop closure likely points towards the same location. %\color{red} -Unsure whether to include following part in this paragraph- \color{black} However, the relative transformation is what multi-robot SLAM intends to find, effectively creating two challenges. Firstly, no estimate of this transformation is initially available. Secondly, a transformation estimate may be wrong if it is based on false inter-robot loop closures. Then, relying on this estimate to select future inter-robot loop closure candidates would only include other false inter-robot loop closures that are consistent with the initial false set, thus creating an unrecoverable belief about the transformation between robots. %In single-robot SLAM information is available on the relative position of the matched scenes. Having such relative position estimates can be of great value to inter-robot loop closures too, but this is a unexplored area because the spatial information is not generally available.  %Hence identifying and rejecting false positive loop closures is critical in perception-aliasing environment. 
%the advance in feature extraction such as \cite{orb-slam}, \cite{semanticlidar} ensures highly efficient computation, two critical problems in front-end usually are not addressed. 

%%%%%%%% Why is this problem challenging? %%%%%%%%%%%
% Despite substantial advances by the SLAM community, multi-robot SLAM remains extremely challenging in practice. Firstly, place recognition identifies scenes that are similar in appearance, but over a longer duration of time, robots may encounter very similar-looking scenes in different locations. In single-robot SLAM, the robot can use odometry data to get a sense of whether the similar scenes are in approximately the same area. However, this odometry backbone does not connect trajectories of different robots in multi-robot SLAM, making it impossible to readily extend this spatial check to multiple robots. Therefore, multi-robot SLAM is sensitive to mismatching scenes, leading to false loop closures. Meanwhile, previous research demonstrates that even a small amount of false loop closures can result in catastrophic failure of the SLAM algorithm \cite{Ikram2022}. 
% A second major challenge is that multi-robot SLAM puts a large strain on computational resources. Reaching real-time execution becomes difficult if a large numbers of potential loop closures are found within a small time-frame. This issue hampers large-scale deployment, because the number of proposed inter-robot loop closures grows with the number of visited places, especially in repetitive environments. 

Despite substantial advances by the SLAM community, finding good inter-robot loop closures remains challenging in practice. First, place recognition identifies scenes that are similar in appearance, but over a longer duration of time, robots may encounter very similar-looking scenes in different locations. Then, these scenes can be mismatched, leading to false inter-robot loop closures. In single-robot SLAM, the robot can use odometry data to get a sense of whether the similar scenes are in approximately the same area. However, this odometry backbone does not connect trajectories of different robots in multi-robot SLAM, making it impossible to readily extend this spatial check to multiple robots. Meanwhile, previous research demonstrates that even a small amount of false loop closures can result in catastrophic failure of the SLAM algorithm \cite{Ikram2022}. 
Second, feeding a large set of (true and false) inter-robot loop closures into the multi-robot SLAM algorithm puts a large strain on computational resources\cite{heavy_loopclousre}. With commonly available robot hardware, reaching real-time execution then becomes difficult. Especially in repetitive environments the number of found inter-robot loop closures grows with the number of visited places, such that this computational bottleneck hampers large-scale deployment. 


%%%%%%%% How does the state of the art approach this challenge? %%%%%%%%%%%
Various existing works tackle the issues of identifying false loop closures and heavy computation. To reject false loop closures, authors of \cite{Mangelson2018} use pairwise consistency maximization (PCM). PCM leverages graph theory to identify the largest set of inter-robot loop closures that are consistent with each other and assumes that this is the true set. However, in repetitive environments this assumption breaks down because a large number of false loop closures can also be consistent with each other. PCM could then accept the set of false inter-robot loop closures instead - a problem often referred to as perceptual aliasing. To solve this problem, authors in \cite{Wang2018} identifies when perceptual aliasing occurs, and keeps track of all different hypotheses. Unfortunately, as a consequence robots have to reason about the best action to take when multiple hypotheses on the environment could be true, which is solved in exponential time with the number of hypotheses \cite{Shienman2022}. %Alternatively, the authors of \cite{Mangelson2018} used pairwise consistency maximization (PCM) to reject false loop closures. Yet, these methods require non-negligible computation power, increasing with the number of loop closures. 
% - Robustness problem: PCM, multiple hypotheses Bayes tree \& planning
% - Resource use problem: compact descriptors, look-up trees (BoW), Bayes tree (iSAM2)
Other researchers instead sought to reduce computation. Loop closure detection speed increased, e.g. due to easily obtainable ORB features for vision-based approaches \cite{ORB}, and efficient look-up trees to match scenes \cite{GalvezLopez2012}. %Additionally, incremental versions exist of PCM \cite{Huang2022} and the optimization procedure to  (iSAM2) \cite{Kaess2012}. 
In \cite{Tian2021b} the authors consider sampling a subset of most informative inter-robot loop closures to reduce overall time consumption. However, the authors also note that the performance guarantee of their sampling method decreases if a scene can be potentially matched to many others - i.e. when there is substantial perceptual aliasing. %However, this would result in missing correct loop closures, thereby losing information that would make the shared situational awareness more accurate and consistent with the real world. %if the number of loop closures to process grows, since the time complexity of the whole pipeline increases with each addition. Furthermore, it happens naturally that more loop closures are found over time, simply because the number of visited places grows. 
% In spite of these advances however, large-scale deployment of multiple robots remains difficult to do in real-time. %The latter reduces computation by editing only the subset of variables affected by newly introduced loop closures, using a Bayes tree. 

%- Both problems: correct place-recognition
% By improving loop closure detection however, researchers have improved robustness and resource use simultaneously. Authors of \cite{Eckehard}, \cite{Erol}, \cite{Egodagamage2018} designed more informative feature extraction algorithms, while authors in \cite{keyposes} focused on selecting a subset of "key" positions (i.e. keyframes) that contain an informative set of features. In \cite{descriptor} the authors designed descriptors to summarize a set of features at each key position \cite{descriptor}. 

% Where do they fall short and what is “the gap” that this paper intends to fill \\

% Stephanie's comments: more on approach and the challenges of this approach
Notably, few researchers have addressed aforementioned problems exploiting relative locations of robots. This spatial information is often assumed unknown in multi-robot SLAM problems. However, we argue that the communication signal itself can be used to retrieve this information by measuring angle-of-arrival (AOA) from phase information and distance from time-of-flight. In our approach \textit{Wi-Closure}, we leverage this spatial information to identify at which positions the trajectories of robots may overlap, as we can presumably only find inter-robot loop closures in these locations. A highly important characteristic of \textit{Wi-Closure} is that it is robust against perceptual aliasing. The method can therefore potentially reject false inter-robot loop closures that would otherwise lead to a failed map or increased computation due to added hypotheses. 
A major challenge to \textit{Wi-Closure} however is multipath propagation of the communication signal, wherein the signal bounces off of various objects to arrive at the receiver from a different angle. Consequently, the AOA measurement may include multiple directions, of which at most one is truly directed towards the other robot. We address this issue by tracking multiple hypotheses, of which the likelihood is iteratively updated using found inter-robot loop closures.   
Our contributions in this paper are as follows:
\begin{enumerate}
    \item We introduce a resource efficient approach, Wi-Closure, to detect loop closures based on spatial information from the communication signal. This approach can be used in tandem with existing similarity-based loop closure detection algorithms.
    \item We address the challenging situation of multi-path propagation of the communication signal using a multiple hypotheses approach.
    \item We demonstrate the merits of our approach in terms of robustness against false inter-robot loop closures and improved computation time by integrating it into the existing frameworks DiSCo-SLAM and Kimera-multi; assessment is done in simulations using the KITTI dataset, and in hardware experiments.
\end{enumerate}

==> Chapters/OLD/2_Related_Work.tex <==
\section{Related Work}

% Add stuff about computation? And sampling method being less robust? Maybe emphasize the computation vs. robustness dilemma in the current literature more
For decades, the majority of research on loop closure detection has been focused on a single robot \cite{GalvezLopez2012,Kin2006}. Recently however, loop closure detection algorithms are being adapted to fleets of robots, to ensure reliable and efficient retrieval of shared map and location estimates \cite{Giamou2018,Mangelson2018}. We leverage previous work on sensing through the communication signal to simultaneously address two open problems in this area: 1) computation to match large trajectories is high, and 2) place recognition can easily mismatch trajectories in repetitive environments. % These methods face two additional challenges in the multi-robot setting, 1) the odometry backbone does not provide any spatial information on the relative position of scenes visited by different robots, and 2) the methods need to be computationally efficient enough to enable real-time collaboration. 
\vspace{4pt}
% Map creation using a single robot has been extensively studied and optimized. However, the area of multi-robot systems for map creation using SLAM is relatively underdeveloped. In single-robot SLAM, odometry measurements are often corrected and used to provide a general map. 
%Furthermore, with the use of multiple robots, accurate loop closure detection becomes increasingly important since robots must know when they have already seen a landmark. 
% \cite{Dennison,DeutschIsaac2016Affm}.

\textbf{Wireless sensing} Extensive research has shown that we can obtain spatial information from wireless signals \cite{Kumar2014AccurateIL}. Many works use UWB sensors to obtain ranging information between two robots by measuring the time-of-flight of the ultra-wideband signal.\cite{uwb_multi1,uwb_multi2} use the ranging information amongst robots to improve the joint position estimate even without being in line of sight of each other. Recently, \cite{Jadhav2021} also introduced sensing direction from the WiFi communication signal to the robotics community, requiring only a single WiFi antenna and movement of the robot. These innovations avoid the need of anchors as used in classical works to estimate position, which come with additional infrastructure that needs to be present in the environment and bulky equipment \cite{classic_position1, classic_position2}. %Instead of using conventional signal strength \cite{signal_strength1,2,3}, it utilizes the motion of robots and attached wifi antennas to emulate antenna arrays in the air to extract bearings without additional infrastructures and bulky equipments. 
% also provide a vision for collaborative robotics to obtain relative spatial information like ranging without relying on the drifting odometers. 
% Source of information rarely incorporated in collaborative robotics. AOA from phase. Distance from ToF or (less accurate) signal strength.\\
% However, the WiFi signal can scatter off various objects, introducing indirect paths between sender and transmitter. This is often referred to as the multipath propagation problem \cite{Vanderveen1998}. Consequently, the AOA measurement can include multiple possible directions, of which maximally one is the true direct path between the two robots. To properly reason about this multipath problem, we can leverage the same frameworks to represent multiple hypotheses as done with repetitive scenes. 

\textbf{Range-only SLAM} Previously, [REFs] used UWB sensors in a multi-robot SLAM setting that has been coined range-only SLAM, where they used the distance measurements directly as inter-robot loop closures. This avoids the problem of perceptual aliasing, but it will only introduce connections between the maps of the robots at locations where the robots are communicating. However, we consider the more realistic situation where communication is intermittent. Then, trajectories could overlap in places where communication is unavailable and where the position estimate is uncertain due to odometer drift. Additional place recognition can then increase the accuracy of the shared map. To our knowledge, we are the first to explicitly speed up place recognition by using ranging and direction information from the communication signal. %%Use as module!!

\textbf{Scene matching} Because of the absence of the odometry backbone, multi-robot SLAM relies on finding inter-robot loop closures. A popular method for this is scene matching, which is often a two-step process, where the first step focuses on checking whether scenes are similar (scene recognition), and the second step will attempt to retrieve a geometric association between the two scenes. A multitude of vision-based methods, such as Kimera-Multi \cite{Tian2021}, DOOR-SLAM \cite{Lajoie2020} and others \cite{Bonin2020,Egodagamage2018,VanOpdenbosch2019}, compress a subset of images (i.e. keyframes) to low dimensional descriptors using e.g. the Bag-of-Words descriptor. Matching these descriptors instead of the images themselves enables low-communication and reliable scene recognition \cite{GalvezLopez2012}. To then retrieve the relative transformation between the two scenes, feature detection algorithms such as SIFT, SURF or ORB extract salient points from each keyframe. These feature points are then processed by computationally intensive methods such as bundle adjustment to retrieve the relative pose information. 
On the other hand, LiDAR based approaches such as DiSCO-SLAM \cite{Huang2022} use different methods in a similar pipeline. Some systems directly extract a descriptor for each LiDAR scan \cite{Huang2022}, and then use iterative closest point (ICP) to retrieve the relative poses of the scans. However, since ICP attempts to fully match the two pointclouds, this method is only able to match LiDAR frames with substantial overlap. To enable scene-matching for LiDAR scans with less overlap, authors from \cite{Zhu2020} first extract semantic information from each scan. With this information they then create histogram-based global descriptors for scene recognition, followed by RANSAC to find a geometrically consistent relative pose.
Lastly, since ICP requires both a good initial guess and substantial computation power, various works focus on replacing ICP by less demanding approaches such as matching planar and line features from LiDAR scans \cite{Lusk2022,Pathak2010,Schaefer2019}. Notably, in both vision-based and LiDAR-based approaches, scene recognition is done by simplifying information-rich measurements into descriptors or semantic information. This loss in information increases the risk of including false loop closures, which can in turn lead to catastrophic optimization failure of the SLAM result \cite{Ikram2022}.\vspace{4pt}
% \subsection{Multi-robot Loop Closure}


% However, using multiple robots increases the complexity of this problem since robots possibly have intermittent wireless connection and limited communication bandwidth. Additionally, in single-robot SLAM the odometry backbone gives an initial guess for the history of poses of the robot, which is further refined by finding loop closures. Such a backbone is not available in multi-robot SLAM, resulting in various disconnected robot trajectories. Therefore, a major issue  

% \textbf{Robustness} In order to increase robustness against false loop closures, researchers have focused on increasing robustness both in the SLAM front-end and back-end. Here, the front-end comprises the processing of raw measurements into low-dimensional estimates of robot and feature poses. In the front-end, RANSAC \cite{Bonin2020,Ikram2022} and PCM \cite{Lusk2022} are often used to reject outlier loop closures. Both methods check whether matched features in a single scene are geometrically consistent with each other, and hence leverage more detailed information from the measurement than the high-level descriptor-matching. In the back-end PCM also plays a significant role. It has become the conventional method to find the largest set of scene matches (i.e. inter-robot loop closures) that give a consistent result, in a dataset where false inter-robot loop closures are present \cite{Mangelson2018}.
%in order to optimize the process of finding loop closure candidates. 
% The intuition of \cite{PCM} is only accepting candidates where the robots are geographically close to each other with geometric consistency metric. 
% The PCM algorithm to estimate the largest set of measurements that are consistent with each other. This set gives the true loop closures, if there is no larger set of consistent false loop closures. 
% However, a critical 
% Alternatively, authors from \cite{Yang2019} used a robust cost-function when optimizing the solution in the SLAM back-end. This approach efficiently integrates outlier-rejection into the optimization problem. Despite reaching impressive performance against outliers however, both methods do not guarantee good performance in repetitive environments. Then, a large set of outliers can be consistent with each other, towards which these methods mistakenly can converge. \vspace{4pt}  %Finding the largest pairwise internally consistent set can be transformed into an instance of the maximum clique problem. While this is known to be an NP-Hard problem, authors of \cite{max_clique} reduce the complexity to $\mathcal{O}(n \cdot \Delta^2)$ where $n$ is the number of vertices in the graph and $\Delta$ is the maximum degree of the graph. The DiSCo-SLAM algorithm uses PCM both; however, they assume that communication is continuous, which is often not true in the real environment. \cite{DiSCo} It would be more beneficial to determine run time while communication occurs intermittently rather than continuously.

\textbf{Repetitive scenes} Although repetitive scenes are pervasive in many environments, classical place recognition approaches find it notoriously difficult to deal with them. Possibly, multiple scenes are similar in appearance, leading to multiple equally likely solutions for matching locations. Therefore, researchers have focused on simultaneously representing all hypotheses in one framework \cite{Hsiao2019}. To properly use these multiple hypotheses to determine the best course of action for the robot, researchers developed data-association belief space planning (DA-BSP) \cite{Pathak2016,Shienman2022}. However, in such ambiguous situations the optimal actions prove to be difficult to compute and the computation time scales exponentially with the amount of hypotheses. Therefore, it is critical to reduce the number of hypotheses as much as possible, in order to enable real-time collaboration. Our approach aims to do this through sensing over the communication signal, such that we can reject similar scenes in different locations \vspace{4pt}

% Potentially, we can get direction and distance measurements from the communication signal itself, as a source of information independent from the SLAM solutions. This requires obtaining AOA and distance

% Research using AOA signals

% Paragraph on multiple hypotheses with AOA

% \subsection{paragraph on inter-robot loop closures}
% Find at least 6 relevant papers\\
% 	--> identify that these inter-robot loop closures are either mutual observation or landmark recognition
	
% \subsection{paragraph on state-of-the art scene recognition (e.g. landmark/feature/descriptor matching)}
% Advances on 1) feature extraction, and 2) descriptor matching (BoW), and 3) feature matching
% Best strategy on how to exchange data for feature matching\\
% 	--> identify robustness a problem
	
% \subsection{paragraph on how methods attempt to improve robustness of scene recognition}
% Front-end: many checks in e.g. ORB-SLAM
% Back-end: PCM or robust cost-functions\\
% 	--> front-end can still be fooled by repetition of high-texture patches, back-end too (adversarial paper)
	


% \subsection{Section on multiple hypotheses methods since we base our approach on these}
% 	- D2A-BSP paper
% 	- Multiple hypotheses Bayes tree\\
% Conclusion : in this paper, we'll use multiple hypotheses to let multipath AOA and aliased feature matching enforce eachother.



% Accurate measurements and loop closure detection are an integral part of multi-robot map creation. Previous works have studied the use of Bag of Words (BoW) to use visualization and feature descriptors in order to identify landmarks. % cite bag of words research papers here
% Some works optimize the map creation process by only having inter-robot communication when robots are geographically close to each other. % cite Distributed trajectory estimation with privacy and communication constraints: a two-stage distributed Gauss-Seidel approach


==> Chapters/OLD/4_Approach.tex <==
\section{Approach}
% \textbf{[Anne: the following focus of the paper would simplify things for us, while maintaining a strong case. What do you think?]} In the least advantageous situation for our method, we have only a single measurement from the communication signal, possibly subject to multipath propagation. Even in this case, we can show substantial improvements of the original algorithm. Throughout the following sections, we will therefore focus on this worst-case scenario to showcase the potential of our approach.
% {\centering\subsection*{-------- Outline --------}
% \vspace{-5mm}
% \textit{\begin{enumerate}
%     \item Matching probability of pose-pair \\
%     - Implementation into MLE 
%     - Given the poses of a pair, what is the matching probability
%     \item Efficiently finding trajectory overlap\\
%     - KD-tree and k-means clustering approach
%     \item Likelihood of the direct path in multipath propagation setting
% \end{enumerate}}
% \subsection*{------ End Outline ------} \par}
% \vspace{5mm}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/Clustering and matching.png}
    \caption{Efficiently finding area's where trajectories overlap.}
    \label{fig:trajectory_overlap_finding}
\end{figure*}

\subsection{Matching probability of pose-pair $(\textbf{x}^\alpha_p, \textbf{x}^\beta_k)$}\label{sec:pose-pair_prob}
A pose-pair $(\textbf{x}^\alpha_p, \textbf{x}_\beta^k)$ is included into set $G$ as a potential inter-robot loop closure, if $p(u_{kp}=1)>p_M$. Notably, this process is repeated for each multipath $P_i\in\mathcal{P}$, resulting in different sets $G_i$ with corresponding $p(u_{kp}|P_i)$. First, solving for the MLE with all local factors $f_\alpha$ and $f_\beta$ and communication factors $f_{comm}^i$ gives the shared pose-graph $\mathcal{T}_i^{\alpha,\beta}$.


% We can model these measurements as stochastic variables with Gaussian noise, and incorporate them into the MLE framework through the factors proposed by \cite{Naseri2019}.
% \begin{align}
%     f^{\alpha,\beta}(\phi|\textbf{x}_\alpha,\textbf{x}_\beta)&= \frac{1}{2\pi I_0(\kappa_{\alpha,\beta})}\exp{(\kappa_{\alpha,\beta}\textbf{u}^T(\phi)\frac{\textbf{x}_\alpha-\textbf{x}_\beta}{\|\textbf{x}_\alpha - \textbf{x}_\beta \|_2})} \cdot \\
%     f^{\alpha,\beta}(d|\textbf{x}_\alpha,\textbf{x}_\beta)&= \frac{1}{\sqrt{2\pi\sigma_{\alpha,\beta}^2}}\exp{(\frac{-1}{\sigma_{\alpha,\beta}} (d-\|\textbf{x}_\alpha - \textbf{x}_\beta \|_2))}
% \end{align}
% where ... 
% We expect that measurements $z_{e,\alpha}^n$ and $z_{e,\beta}^k$ can only contain inter-robot loop closures if they are positioned near each other. Therefore, now that the two trajectories $\mathcal{T}_\alpha$ and $\mathcal{T}_\beta$ are connected through the wireless measurements, %we are able to determine this.% if two robot positions $\textbf{x}_\alpha^{n}:\ T_\alpha \in \mathcal{T}_\alpha$ and $\textbf{x}_\beta^k:\ T_\beta\in \mathcal{T}_\beta$ are nearby each other.  Therefore, only the measurements from that specific pose-pair need to be sent and processed. 
% the problem becomes finding the set $G$ of pose-pairs that are within some range of each-other. 
% \begin{align}\label{eq:problem_groundtruth}
%     G = \{\textbf{x}_\alpha^{n} \in \chi_\alpha ,\textbf{x}_\beta^k \in \chi_\beta : ||\textbf{x}_\alpha^n - \textbf{x}_\beta^k|| \leq D \} 
% \end{align}
% where $D$ is a user parameter that determines when two positions are considered to be sufficiently close. This parameter reflects the maximum range of the sensing modality, e.g. camera or LiDAR. Tuning this parameter will have effect on the trade-off between the amount of missed inter-robot loop closures (false negatives) and the amount of falsely included inter-robot loop closure candidates (false positives).

% Different factor types:
% \begin{align}
%     &f_i(z_i, u_i | \textbf{x}_i, \textbf{x}_{i+1}) = f_i(z_i | \textbf{x}_i, \textbf{x}_{i+1})f_i(u_i | \textbf{x}_i, \textbf{x}_{i+1}) \\ &\quad = \frac{1}{4\pi^2|\Sigma|^2}e^{-\frac{1}{2}\|z_i - \textbf{x}_{i+1} + \textbf{x}_i \|_{\Sigma_i}-\frac{1}{2}\|x_{i+1} - A\textbf{x}_{i} + B\textbf{u}_i \|_{\Sigma_i}}\\
%     % &f^{\alpha,\beta}(\phi,d|\textbf{x}_\alpha,\textbf{x}_\beta)=\\
%     % &\quad\frac{1}{2\pi I_0(\kappa_{\alpha,\beta})}\exp{(\kappa_{\alpha,\beta}\textbf{u}^T(\phi)\frac{\textbf{x}_\alpha-\textbf{x}_\beta}{\|\textbf{x}_\alpha - \textbf{x}_\beta \|_2})} \cdot \\
%     % &\quad \frac{1}{\sqrt{2\pi\sigma_{\alpha,\beta}^2}}\exp{(\frac{-1}{\sigma_{\alpha,\beta}} (d-\|\textbf{x}_\alpha - \textbf{x}_\beta \|_2))}
% \end{align}

% Reduces to LSQ\\

\begin{align}
    \mathcal{L}^i =&  \prod_{k}f^i_{comm,k}(\phi_k,d_k|\mathcal{T}^{\alpha,\beta}_i) \cdot \\ &\prod_{l}f_{\alpha,l}(z_l|\mathcal{T}^{\alpha,\beta}_i) \prod_{m}f_{\beta,m}(z_m|\mathcal{T}^{\alpha,\beta}_i)
\end{align}
Then, for each pose-pair $(\textbf{x}_p^\alpha,\textbf{x}_k^\beta)$ we calculate covariance matrix $\Sigma^i_{kp}$ with
\begin{align}
    % \Bar{\textbf{x}}^\alpha_{i,j} &= \textbf{x}_{p}^\alpha - R^\alpha_\beta\textbf{x}_{k}^\beta,\quad \textbf{x}_{p}^\alpha, \textbf{x}_{k}^\beta\in\mathcal{T}^{\alpha,\beta}_i \\
    \Sigma^i_{kp} 
    % &= [\mathcal{I}^i_{j}]^{-1} \\
    &= \left(-E\left[\frac{\partial^2 \log \mathcal{L}^i  }{\partial \textbf{x}^p_k \partial\textbf{x}^p_k}\right]\right)^{-1}
\end{align}

Using equation \ref{eq:prob_true_LC}, we can now compute $p(u_{kp}|P_i)$ for each pose-pair $(\textbf{x}_p^\alpha,\textbf{x}_k^\beta)$ and each multipath $P_i\in\mathcal{P}$. 

\subsection{Efficiently finding trajectory overlap}
Rather than comparing for all possible pose-pairs $\textbf{x}^\alpha_p\in\mathcal{T}^\alpha$ and $\textbf{x}^\beta_k\in\mathcal{T}^\beta$ if they are positioned close to each other, we aim to find an efficient method to initially find where trajectories of the robots overlap. After the initial search in this section, the selection of pose-pairs is further narrowed down to find set $G$ with the method previously described in Section \ref{sec:pose-pair_prob}.\\


% Intuitively, our approach bounds the area covered by some robot $A$, and then queries where this area overlaps with robot $B$'s trajectory. Next, robot $B$ bounds the found overlap similarly by some area, and queries which part of robot $A$'s trajectory overlaps. Lastly, robot $A$ subdivides the part of its trajectory that may have overlap with robot $B$, and then repeats the process. 
As shown in Figure \ref{fig:trajectory_overlap_finding}, our approach first bounds the area's traversed by robots $A$ and $B$, and selects the poses where these bounds overlap. Then, the poses in the overlapping area are divided into clusters using $k$-means clustering, and the process is repeated for each found cluster. 

The initial bounds on the area are found simply by selecting the minimum and maximum position coordinate along each dimension. However, we need to add an additional distance $d_{buffer}$ to these bounds to account for possible distance between true loop closures (Equation \ref{eq:prob_trueLC_given_pose}) and uncertainty in the poses (Equation \ref{eq:prob_poses}). After adding $d_{buffer}$ to the initial bounds, the bounded area should contain the whole trajectory of robot $A$ (or $B$) at a $\gamma\%$-confidence level, with respect to any pose in robot $B$'s (or $A$'s) trajectory. For this, we first define an upper bound on the worst-case uncertainty $\sigma_{max}$ of the translation $\textbf{x}^p_k$ between any two poses $\textbf{x}^\alpha_{p}\in\mathcal{T}^{\alpha}$ and $\textbf{x}^\beta_{k}\in\mathcal{T}^{\beta}$. 
% Use $\mathcal{T}^{\alpha,\beta}$. Bound position of $\mathcal{T}^{\alpha}$ by $\textbf{x}^\alpha_{min} = \min_{\textbf{x}^\alpha_{p}}(\mathcal{T}^{\alpha})$ and $\textbf{x}^\alpha_{max} = \max_{\textbf{x}^\alpha_{p}}(\mathcal{T}^{\alpha})$. Query to robot B whether any of robot B's poses lie within this region plus some buffer $d_{buffer}$ to account for uncertainty. Here, this uncertainty buffer is an upper bound on worst-case uncertainty $\sigma_{max}$ of the translation $\textbf{x}^p_k$ between any two poses $\textbf{x}^\alpha_{p}\in\mathcal{T}^{\alpha}$ and $\textbf{x}^\beta_{k}\in\mathcal{T}^{\beta}$. 
\begin{align}
    \sigma_{max}^2 = \max_{k,p}( \lambda_{max} (\Sigma_{kp})), \quad p,k\in t
\end{align}
where $\lambda_{max}$ is the largest eigenvalue of $\Sigma_{kp}$. Then, we rewrite $\textbf{x}^p_k$ in terms of the local frames.
\begin{align}
    \textbf{x}^p_k% = \textbf{x}^\alpha_p - T^\alpha_\beta\textbf{x}^\beta_k
    = \underbrace{\textbf{x}^\alpha_p  - (\textbf{x}^\alpha_\beta + R^\alpha_\beta \textbf{x}^\beta_k)}_{RH}
\end{align}
Dropping the correlations between the three terms in $RH$ will give an upperbound on $\lambda_{max}(\Sigma_{kp})$, i.e.
\begin{align*}
    \lambda_{max}(\Sigma_{kp}) &\leq \lambda_{max}(\Sigma_{kp}^{RH}) \\
    &= \lambda_{max}(\Sigma_{\alpha p} + J_{\alpha\beta}^T \Sigma_{\alpha\beta}J_{\alpha\beta} + J_{\beta k}^T \Sigma_{\beta k}J_{\beta k})
\end{align*}
Then, we can further split this term.
\begin{align*}
    \lambda_{max}(\Sigma_{kp}^{RH}) %&= \lambda_{max}(\Sigma_{\alpha p} + J_{\alpha\beta}^T \Sigma_{\alpha\beta}J_{\alpha\beta} + J_{\beta k}^T \Sigma_{\beta k}J_{\beta k}) \\
    &\leq \lambda_{max}(\Sigma_{\alpha p}) + \lambda_{max}(J_{\alpha\beta}^T \Sigma_{\alpha\beta}J_{\alpha\beta}) \\&\quad + \lambda_{max}(J_{\beta k}^T \Sigma_{\beta k}J_{\beta k})\\
    &= \lambda_{kp}^{UB}
\end{align*}
where $J_{\alpha\beta}$ is the Jacobian of $\textbf{x}_{\alpha\beta}$, and $J_{\beta k}$ the Jacobian of $R^\alpha_\beta \textbf{x}^\beta_k$. This formulation allows for distributed computation of $\sigma_{UB}$ as an upper bound to $\sigma_{max}$.
\begin{align*}
    \sigma_{UB}^2 &= \max_{k,p\in t}( \lambda_{kp}^{UB} )\\
    &= \max_{p\in t}( \lambda_{max}(\Sigma_{\alpha p})) + \lambda_{max}(J_{\alpha\beta}^T \Sigma_{\alpha\beta}J_{\alpha\beta}) \\&\quad + \max_{k\in t}(\lambda_{max}(J_{\beta k}^T \Sigma_{\beta k}J_{\beta k}) ))\\
    &\geq \max_{k,p}( \lambda_{max} (\Sigma_{kp})) = \sigma_{max}^2
\end{align*}
Lastly, we combine $\sigma_{UB}$ and $c^{-1}$ - the variance of the distance between true loop closures as in Equation \ref{eq:prob_trueLC_given_pose} - to retrieve $d_{buffer}$.
\begin{equation}
    d_{buffer} = z_\gamma \sqrt{\sigma_{UB}^2 + c^{-1}}
\end{equation}
where $z_\gamma$ is the number of standard deviations needed to achieve at least $\gamma\%$-confidence level.
% Then, all poses that are included by robot B are bounded in a similar way, and robot B queries robot A whether any of robot A's poses are within this area. Lastly, we split the poses found by robot A into multiple clusters, and repeat the process.
\\

% Select some pose $\textbf{x}^k_\alpha\in\mathcal{X}_\alpha$ and $\textbf{x}^p_\beta\in\mathcal{X}_\beta$. Then, we can define the uncertainty of any pose $\textbf{x}^t_\alpha\in\mathcal{X}_\alpha$ w.r.t. $\textbf{x}^k_\alpha$ by some uncertainty ellipsoid $\mathcal{E}^{t,k}_\alpha$ that indicates the uncertainty in the relative location with $\gamma$\% confidence. The worst-case uncertainty of any $\textbf{x}^t_\alpha\in\mathcal{X}_\alpha$ w.r.t. $\textbf{x}^k_\alpha$ is bounded by the minimum volume ellipsoid $\mathcal{E}^{max,k}_\alpha$ that covers the union of zero-centered uncertainty ellipsoids $\mathcal{E}^{0,k}_\alpha,\dots,\mathcal{E}^{\tau,k}_\alpha$. We can calculate $\mathcal{E}^{max,k}_\alpha$, and similarly  $\mathcal{E}^{max,k}_\beta$ efficiently with a convex semidefinite program \cite{boyd_vandenberghe_2009}, and return corresponding worst-case covariance matrices $\Sigma_\alpha^{max,k}$ and $\Sigma_\beta^{max,p}$.

% Additionally, we retrieve the covariance matrix $\Sigma^{k,p}$ between poses $\textbf{x}^k_\alpha\in\mathcal{X}_\alpha$ and $\textbf{x}^p_\beta\in\mathcal{X}_\beta$ from the MLE.

% The transformation between pose $\textbf{x}^{t_1}_\alpha\in\mathcal{X}_\alpha$ and $\textbf{x}^{t_2}_\beta\in\mathcal{X}_\beta$ can be achieved by the following smaller transformations
% \begin{align}
%     \textbf{x}^{t_1,t_2}_{\alpha,\beta} = \textbf{x}^{t_2,p}_\beta \oplus \textbf{x}^{p,k}_{\alpha,\beta} \oplus \textbf{x}^{k,t_1}_\alpha
% \end{align}

% Therefore, worst case uncertainty represented by covariance matrix $\Sigma^{max}$ between any pose-pair $(\textbf{x}_\alpha\in\mathcal{X}_\alpha, \textbf{x}_\beta\in\mathcal{X}_\beta)$ is bounded by the combined uncertainty of $\Sigma_\alpha^{max,k}$, $\Sigma_\beta^{max,p}$ and $\Sigma^{k,p}$: \textit{see paper https://arxiv.org/pdf/1906.07795v1.pdf for how to combine uncertainty matrices}.

% From $\Sigma^{max}$ with largest eigenvalue $\lambda_1$ and corresponding eigenvector $v_1$, we can derive the size of the uncertainty buffer $d_{buffer}$ in Figure \ref{fig:trajectory_overlap_finding} as follows
% \begin{align}
%     d_{buffer,x} &= (\lambda_1 \textbf{v}_1 \cdot \begin{bmatrix}1 \\ 0\end{bmatrix}+c)\chi_\gamma\\
%     d_{buffer,y} &= (\lambda_1 \textbf{v}_1 \cdot \begin{bmatrix}0 \\ 1\end{bmatrix}+c)\chi_\gamma
% \end{align}
% where $\cdot$ denotes the inproduct, $c$ is the variance of the Gaussian mapping $(\textbf{x}_\alpha,\textbf{x}_\beta)_{kp} \to p(u_{kp})$, and $\chi_\gamma$ denotes the confidence level of $d_{buffer}$.




\subsection{Identifying direct path in a multipath propagation setting}
% The communication signal can arrive at the robot via $n$ different propagation paths, which form the set of binary variables $\mathcal{P}=\{P_1, P_2, ...,P_n \}$. Here, $P_i=1$ indicates that path $i$ is the direct path. We capture this multipath propagation phenomena in the AOA measurement by modeling this measurement as a multimodal variable, such that $f(\phi)$ is the marginal distribution of multiple Gaussian distributions.
% \begin{align}
%     f(\phi) &= \sum_i^{|\mathcal{P}|} 
%     f^{\alpha,\beta} (\phi | P_i)p(P_i)
% \end{align}
% Each mode $ f^{\alpha,\beta} (\phi | P_i)$ with $P_i\in\mathcal{P}$ results in a different MLE estimate of the poses $\hat{\mathcal{X}}_i$, where we denote the optimized MLE estimate with a hat. We retrieve the MLE estimates of each mode by replacing $f^{\alpha,\beta}(\phi| \textbf{x}_\alpha, \textbf{x}_\beta)$ in equation \ref{eq:MLE} with the Gaussian distribution $f^{\alpha,\beta}(\phi|P_i, \textbf{x}_\alpha, \textbf{x}_\beta)$. Finally, for each $\hat{\mathcal{X}}_i$, we search for the set of candidate inter-robot loop closures $G_\Sigma^i$ (as previously defined in the Problem Statement).
% \begin{align}
%     G_\Sigma^i = \{... | \hat{\mathcal{X}}_i\}
% \end{align}

% Each of the pose-pairs in candidate set $G_\Sigma^i$ is either a true or false loop-closure. Let us define the binary variable $u_{kp}$ for each pose-pair $(\textbf{x}^i_\alpha, \textbf{x}^i_\beta)_{kp}\in G_\Sigma^i$, such that $u_{kp}=1$ if pose-pair $(\textbf{x}^i_\alpha, \textbf{x}^i_\beta)_{kp}$ is a true loop-closure, and $u_{kp}=0$ otherwise. 
Our algorithm will only find correct inter-robot loop closures if the AOA measurement captures the direct path. However, due to the multipath problem, we have a set $\mathcal{P}$ of which maximally one path is the direct path. In this section we show how to apply Bayes rule to provide the probability of some path $P_i\in\mathcal{P}$ being the direct path. \\

First, for a number of inter-robot loop closures $(\textbf{x}^\alpha_p, \textbf{x}^\beta_k)\in G_i$, we check whether they are a match e.g. by applying ICP, bundle adjustment or PCM. This thus provides us with the information $u_{kp}=U_{kp}$ with $U_{kp}=1$ for a successfull match, and $U_{kp}=0$ if the match is rejected. Given the new information, we can update the probability of $P_i$ being the true direct path with Bayes rule.
\begin{align}
    % f(\phi | \textbf{u}) &= \sum_i^{|\mathcal{P}|} f^{\alpha,\beta} (\phi | P_i) \underbrace{p(P_i|u_{kp})}_{w_i(u_{kp})}\\
    % &=\sum_i^{|\mathcal{P}|} f^{\alpha,\beta} (\phi | P_i)\frac{p(u_{kp}|P_i)p(P_i)}{p(u_{kp})}
    p(P_i|u_{kp}=U_{kp}) = \frac{p(u_{kp}=U_{kp}|P_i)p(P_i)}{p(u_{kp}=U_{kp})}
\end{align}
where $p(u_{kp}=U_{kp}|P_i)$ is computed as in equation \ref{eq:prob_true_LC}, $p(P_i)$ is the prior, and $p(u_{kp})$ is some normalization constant such that $\sum_{P_i\in\mathcal{P}}p(P_i|u_{kp})=1$.\\

% We re-use previously defined relations under each hypothesis that path $P_i$ is the true direct path. Thus, the probability that pose-pair $(\textbf{x}_k^\alpha, \textbf{x}_p^\beta)$ is a true inter-robot loop closure, is given by
% ------------------- Mahalanobis method -------------------\\
% \begin{align}
%     p(u_{kp}| P_i, \textbf{x}_p^{\alpha}, \textbf{x}_k^{\beta} ) &= e^{\ - \frac{1}{2}c\| \textbf{x}_p^{\alpha}-\textbf{x}_k^{\beta} \|_2 },\quad c>0\\
% \end{align}
% We can use the same result from Eq. \ref{eq:prob_true_LC} to obtain $p(u_{kp}|P_i)$ by marginalizing over the positions of the pose-pair. The only difference is that we now have an additional conditional dependency on $P_i$ being the true path.
% \begin{align}
%     p(u_{kp} | P_i) &= \int_{\mathbb{R}^d} p(u_{kp} | P_i, (\textbf{x}^i_{\alpha}, \textbf{x}^i_{\beta})_{kp}) f((\textbf{x}^i_{\alpha}, \textbf{x}^i_{\beta})_{kp}|P_i)dx\\
%     % &= \int_{\mathbb{R}^d} e^{\ - \frac{1}{2}c\| \textbf{x}^i_{\alpha,j}-\textbf{x}^i_{\beta,j} \|_2 -\frac{1}{2}\| \Bar{\textbf{x}}+\textbf{x}^i_{\alpha,j}-\textbf{x}^i_{\beta,j} \|_{\Sigma^{-1}}}dx\\
%     % &= e^{-\frac{1}{2}\Bar{\textbf{x}}\Sigma^{-1}\Bar{\textbf{x}}}\int_{\mathbb{R}^d} e^{\ -\frac{1}{2} \textbf{D}^T (\Sigma^{-1} + cI) \textbf{D} - \Bar{\textbf{x}}^T\Sigma^{-1}\textbf{D}}dx\\
%     % &=\sqrt{\frac{(2\pi)^d}{\det (\Sigma^{-1} +cI)}}e^{-\frac{1}{2}\Bar{\textbf{x}}^T\Sigma^{-1}\Bar{\textbf{x}} + \Bar{\textbf{x}}^T\Sigma^{-1} (\Sigma^{-1} +cI)^{-1}\Sigma^{-1}\Bar{\textbf{x}}}
% \end{align}

% ------------------- Binomial method -------------------\\
% If propagation path $P_i$ truly is the direct path, then we expect a large proportion of the pose-pairs in $G_\Sigma^i$ to be true loop-closures, i.e. a large true positive rate (TP).
% \begin{align}
%     E_{kp}[u_{kp}| P_i=1] = TP
% \end{align}
% Meanwhile, if propagation path $P_i$ is not the direct path, there are likely less loop-closures. Therefore, we can use hypothesis testing to compute the probability of observing $m$ true loop closures in $G_\Sigma^i$, given the poses $\mathcal{X}_i$.
% \begin{align}
%     % H_0:\ &E_{kp}[u_{kp} | P_i=1] = TP\\
%     % H_1:\ &E_{kp}[u_{kp} | P_i=0] < TP
%     H_0:\ &p(u_{kp}=1) = TP\\
%     H_1:\ &p(u_{kp}=1) < TP
% \end{align}
% Variable $u_{kp}$ follows the binomial distribution, such that the probability of having $k_b$ true loop closures in a set of $n_b$ loop closure candidates is given by
% \begin{align}
%     P(u_{kp}=k_b)=\begin{pmatrix}n_b \\k_b \end{pmatrix}TP^{k_b} (1-TP)^{n_b-k_b}
% \end{align}
% Hypothesis $H_0$ is then rejected if $P(u_{kp} \leq k_b|P_i=1) \leq \gamma$. \\
% ---------------------------------------------------------------------\\


% For each MLE solution, we can define for any pair of poses $(\hat{\textbf{x}}_{\alpha,i}^k, \hat{\textbf{x}}_{\beta,i}^p)$, the pdf of the distance between these poses, and the corresponding probability $p( \hat{\textbf{x}}_{\alpha,i}^k - \hat{\textbf{x}}_{\beta,i}^p |\ u=1)$.

% \begin{align}
%     f(\hat{\textbf{x}}_{\alpha,i}^k - \hat{\textbf{x}}_{\beta,i}^p) = c e^{ -\frac{1}{2}\| \hat{\textbf{x}}_{\alpha,i}^k - \hat{\textbf{x}}_{\beta,i}^p \|_\Sigma}
% \end{align}
% Then, the probability that a pair of poses are actually in the same position is
% -----------------------------
% \begin{align}
%     f(\phi|\textbf{x}_\alpha,\textbf{x}_\beta)&= \sum_i^{|\mathcal{P}|} 
%     f^{\alpha,\beta}(\phi | P_i, \textbf{x}_\alpha,\textbf{x}_\beta) \underbrace{p(P_i | \textbf{x}_\alpha,\textbf{x}_\beta)}_{w_i}\\
%     % f^{\alpha,\beta}(\phi,P_i |\textbf{x}_\alpha,\textbf{x}_\beta) \\%\underbrace{p(P_i | \textbf{x}_\alpha,\textbf{x}_\beta)}_{w_i}
%     w_i&= \frac{f(\textbf{x}_\alpha,\textbf{x}_\beta | P_i)p(P_i)}{f(\textbf{x}_\alpha,\textbf{x}_\beta)}\\
%     % w_i f^{\alpha,\beta}(\phi_i | \textbf{x}_\alpha,\textbf{x}_\beta) \\
%     \sum_i w_i &= 1 % Direct path not necessarily in here
% \end{align}
% % Assumption: one of the paths is the direct path.
% Relation between propagation path and pose matches.
% % \begin{align}
% %     f^{\alpha,\beta}(\phi|\textbf{x}_\alpha,\textbf{x}_\beta, u)&=f^{\alpha,\beta}(\phi|\textbf{x}_\alpha,\textbf{x}_\beta)f(\textbf{x}_\alpha,\textbf{x}_\beta|u) 
% % \end{align}
% \begin{align}
%     p(P_i | u=U) &= \int_{\mathbb{R}^d} p(P_i | \textbf{x}_\alpha,\textbf{x}_\beta) f(\textbf{x}_\alpha,\textbf{x}_\beta|u=U)dx\\
%     &=p(P_i)\int_{\mathbb{R}^d} \frac{f(\textbf{x}_\alpha,\textbf{x}_\beta | P_i)}{f(\textbf{x}_\alpha,\textbf{x}_\beta)} f(\textbf{x}_\alpha,\textbf{x}_\beta|u=U)dx\\
%     E_u[p(P_i | u&=U)] = p(U_0)p(P_i | u=U_0) \\ &\qquad+ p(U_1)p(P_i | u=U_1)
% \end{align}

Alternatively, %instead of passively updating the probability that some $P_i\in\mathcal{P}$ is the direct path, 
we can actively plan which pose-pairs would provide the most information to differentiate between direct and indirect paths. For this, we minimize Shannon entropy $J = -\sum_i w_i\log (w_i)$, with $w_i = p(P_i)=E_u[p(P_i|u_{kp})]$.
\begin{align}
    \hat{u}_{kp} &= \arg\min_{u_{kp}\in G_{tot}} J(u_{kp})
\end{align}
We narrow the search-space for $u_{kp}$ to $G_{tot}$, which is the union of all $G_i$. After all, inter-robot loop closures that are not part of any $G_i$ are not likely to contain much information on which set $G_i$ corresponds to the true direct path $P_i=1$.

==> Chapters/OLD/4_Approach_V2.tex <==
\section{Approach}
This section explains the approach taken by \textit{Wi-Closure} on three core aspects. The first part shows how trajectory information and communication measurements are used to determine if some position-pair is a candidate inter-robot loop closure. However, determining this for each possible pair of positions has complexity $\mathcal{O}(mn)$, if the trajectories consist of $m$ and $n$ positions respectively. Therefore, in the second section we introduce an algorithm akin the classical branch-and-bound algorithm to quickly find clusters of position-pairs. Lastly, the previously introduced components only work if the communication measurements do not include multipath. Therefore, the third part of this section presents how PCM can be used to identify a set of direct paths from the multipath AOA measurements. 

% {\centering\subsection*{-------- Outline --------}
% \vspace{-5mm}
% \textit{\begin{enumerate}
%     \item Matching probability of pose-pair \\
%     - Implementation into MLE 
%     - Given the poses of a pair, what is the matching probability
%     \item Efficiently finding trajectory overlap\\
%     - KD-tree and k-means clustering approach
%     \item Likelihood of the direct path in multipath propagation setting
% \end{enumerate}}
% \subsection*{------ End Outline ------} \par}
% \vspace{5mm}

\begin{figure*}[b]
    \centering
    \includegraphics[width=\linewidth]{Figures/Clustering and matching.png}
    \caption{Efficiently finding area's where trajectories overlap.}
    \label{fig:trajectory_overlap_finding}
\end{figure*}

% \subsection{Matching probability of pose-pair $(\textbf{x}^\alpha_p, \textbf{x}^\beta_k)$}\label{sec:pose-pair_prob}
\subsection{Trajectories $\mathcal{T}^{\alpha,\beta}$ through sensing via communication}
% A pose-pair $(\textbf{x}^\alpha_p, \textbf{x}_\beta^k)$ is included into set $G$ as a potential inter-robot loop closure, if $p(u_{kp}=1)>p_M$. 
The first step in our approach is to retrieve the shared pose-graph $\mathcal{T}^{\alpha,\beta}$ based on measurements from the odometer and communication signal. The difficulty here is if AOA measurements from the communication signal contain multiple modes. Each communication measurement $f_{multi}^t$ at time $t$ then has a set of paths $P_i\in\mathcal{P}_t$ of which one path may refer to the direct path between the robots. We need to select a single path for each communication measurement to compute the MLE estimate of $\mathcal{T}^{\alpha,\beta}$. For $N_c$ communication measurements, we collect the indices $i$ of the selected paths $P_i$ in combination vector $\mathcal{C}\in \mathbb{N}^{N_c}$.


\begin{align}
    \mathcal{L}^\mathcal{C} =&  \prod_{k=1}^{N_c}f^{\mathcal{C}(k)}_{comm,k}(\phi_k,d_k|\mathcal{T}^{\alpha,\beta}_{\mathcal{C}}, P_{\mathcal{C}(k)}) \cdot \\ &\prod_{l}f_{\alpha,l}(z_l|\mathcal{T}^{\alpha,\beta}_i) \prod_{m}f_{\beta,m}(z_m|\mathcal{T}^{\alpha,\beta}_i)
\end{align}
Then, for each pose-pair $(\textbf{x}_p^\alpha,\textbf{x}_k^\beta)$ we calculate covariance matrix $\Sigma^i_{kp}$ with
\begin{align}
    % \Bar{\textbf{x}}^\alpha_{i,j} &= \textbf{x}_{p}^\alpha - R^\alpha_\beta\textbf{x}_{k}^\beta,\quad \textbf{x}_{p}^\alpha, \textbf{x}_{k}^\beta\in\mathcal{T}^{\alpha,\beta}_i \\
    \Sigma^i_{kp} 
    % &= [\mathcal{I}^i_{j}]^{-1} \\
    &= \left(-E\left[\frac{\partial^2 \log \mathcal{L}^i  }{\partial \textbf{x}^p_k \partial\textbf{x}^p_k}\right]\right)^{-1}
\end{align}

Using equation \ref{eq:prob_true_LC}, we can now compute $p(u_{kp}|P_i)$ for each pose-pair $(\textbf{x}_p^\alpha,\textbf{x}_k^\beta)$ and each multipath $P_i\in\mathcal{P}$. 

\subsection{Efficiently finding trajectory overlap}
Rather than comparing for all possible pose-pairs $\textbf{x}^\alpha_p\in\mathcal{T}^\alpha$ and $\textbf{x}^\beta_k\in\mathcal{T}^\beta$ if they are positioned close to each other, we aim to find an efficient method to initially find where trajectories of the robots overlap. After the initial search in this section, the selection of pose-pairs is further narrowed down to find set $G$ with the method previously described in Section \ref{sec:pose-pair_prob}.\\


% Intuitively, our approach bounds the area covered by some robot $A$, and then queries where this area overlaps with robot $B$'s trajectory. Next, robot $B$ bounds the found overlap similarly by some area, and queries which part of robot $A$'s trajectory overlaps. Lastly, robot $A$ subdivides the part of its trajectory that may have overlap with robot $B$, and then repeats the process. 
As shown in Figure \ref{fig:trajectory_overlap_finding}, our approach first bounds the area's traversed by robots $A$ and $B$, and selects the poses where these bounds overlap. Then, the poses in the overlapping area are divided into clusters using $k$-means clustering, and the process is repeated for each found cluster. 

The initial bounds on the area are found simply by selecting the minimum and maximum position coordinate along each dimension. However, we need to add an additional distance $d_{buffer}$ to these bounds to account for possible distance between true loop closures (Equation \ref{eq:prob_trueLC_given_pose}) and uncertainty in the poses (Equation \ref{eq:prob_poses}). After adding $d_{buffer}$ to the initial bounds, the bounded area should contain the whole trajectory of robot $A$ (or $B$) at a $\gamma\%$-confidence level, with respect to any pose in robot $B$'s (or $A$'s) trajectory. For this, we first define an upper bound on the worst-case uncertainty $\sigma_{max}$ of the translation $\textbf{x}^p_k$ between any two poses $\textbf{x}^\alpha_{p}\in\mathcal{T}^{\alpha}$ and $\textbf{x}^\beta_{k}\in\mathcal{T}^{\beta}$. 
% Use $\mathcal{T}^{\alpha,\beta}$. Bound position of $\mathcal{T}^{\alpha}$ by $\textbf{x}^\alpha_{min} = \min_{\textbf{x}^\alpha_{p}}(\mathcal{T}^{\alpha})$ and $\textbf{x}^\alpha_{max} = \max_{\textbf{x}^\alpha_{p}}(\mathcal{T}^{\alpha})$. Query to robot B whether any of robot B's poses lie within this region plus some buffer $d_{buffer}$ to account for uncertainty. Here, this uncertainty buffer is an upper bound on worst-case uncertainty $\sigma_{max}$ of the translation $\textbf{x}^p_k$ between any two poses $\textbf{x}^\alpha_{p}\in\mathcal{T}^{\alpha}$ and $\textbf{x}^\beta_{k}\in\mathcal{T}^{\beta}$. 
\begin{align}
    \sigma_{max}^2 = \max_{k,p}( \lambda_{max} (\Sigma_{kp})), \quad p,k\in t
\end{align}
where $\lambda_{max}$ is the largest eigenvalue of $\Sigma_{kp}$. Then, we rewrite $\textbf{x}^p_k$ in terms of the local frames.
\begin{align}
    \textbf{x}^p_k% = \textbf{x}^\alpha_p - T^\alpha_\beta\textbf{x}^\beta_k
    = \underbrace{\textbf{x}^\alpha_p  - (\textbf{x}^\alpha_\beta + R^\alpha_\beta \textbf{x}^\beta_k)}_{RH}
\end{align}
Dropping the correlations between the three terms in $RH$ will give an upperbound on $\lambda_{max}(\Sigma_{kp})$, i.e.
\begin{align*}
    \lambda_{max}(\Sigma_{kp}) &\leq \lambda_{max}(\Sigma_{kp}^{RH}) \\
    &= \lambda_{max}(\Sigma_{\alpha p} + J_{\alpha\beta}^T \Sigma_{\alpha\beta}J_{\alpha\beta} + J_{\beta k}^T \Sigma_{\beta k}J_{\beta k})
\end{align*}
Then, we can further split this term.
\begin{align*}
    \lambda_{max}(\Sigma_{kp}^{RH}) %&= \lambda_{max}(\Sigma_{\alpha p} + J_{\alpha\beta}^T \Sigma_{\alpha\beta}J_{\alpha\beta} + J_{\beta k}^T \Sigma_{\beta k}J_{\beta k}) \\
    &\leq \lambda_{max}(\Sigma_{\alpha p}) + \lambda_{max}(J_{\alpha\beta}^T \Sigma_{\alpha\beta}J_{\alpha\beta}) \\&\quad + \lambda_{max}(J_{\beta k}^T \Sigma_{\beta k}J_{\beta k})\\
    &= \lambda_{kp}^{UB}
\end{align*}
where $J_{\alpha\beta}$ is the Jacobian of $\textbf{x}_{\alpha\beta}$, and $J_{\beta k}$ the Jacobian of $R^\alpha_\beta \textbf{x}^\beta_k$. This formulation allows for distributed computation of $\sigma_{UB}$ as an upper bound to $\sigma_{max}$.
\begin{align*}
    \sigma_{UB}^2 &= \max_{k,p\in t}( \lambda_{kp}^{UB} )\\
    &= \max_{p\in t}( \lambda_{max}(\Sigma_{\alpha p})) + \lambda_{max}(J_{\alpha\beta}^T \Sigma_{\alpha\beta}J_{\alpha\beta}) \\&\quad + \max_{k\in t}(\lambda_{max}(J_{\beta k}^T \Sigma_{\beta k}J_{\beta k}) ))\\
    &\geq \max_{k,p}( \lambda_{max} (\Sigma_{kp})) = \sigma_{max}^2
\end{align*}
Lastly, we combine $\sigma_{UB}$ and $c^{-1}$ - the variance of the distance between true loop closures as in Equation \ref{eq:prob_trueLC_given_pose} - to retrieve $d_{buffer}$.
\begin{equation}
    d_{buffer} = z_\gamma \sqrt{\sigma_{UB}^2 + c^{-1}}
\end{equation}
where $z_\gamma$ is the number of standard deviations needed to achieve at least $\gamma$-confidence level.
% Then, all poses that are included by robot B are bounded in a similar way, and robot B queries robot A whether any of robot A's poses are within this area. Lastly, we split the poses found by robot A into multiple clusters, and repeat the process.
\\

% Select some pose $\textbf{x}^k_\alpha\in\mathcal{X}_\alpha$ and $\textbf{x}^p_\beta\in\mathcal{X}_\beta$. Then, we can define the uncertainty of any pose $\textbf{x}^t_\alpha\in\mathcal{X}_\alpha$ w.r.t. $\textbf{x}^k_\alpha$ by some uncertainty ellipsoid $\mathcal{E}^{t,k}_\alpha$ that indicates the uncertainty in the relative location with $\gamma$\% confidence. The worst-case uncertainty of any $\textbf{x}^t_\alpha\in\mathcal{X}_\alpha$ w.r.t. $\textbf{x}^k_\alpha$ is bounded by the minimum volume ellipsoid $\mathcal{E}^{max,k}_\alpha$ that covers the union of zero-centered uncertainty ellipsoids $\mathcal{E}^{0,k}_\alpha,\dots,\mathcal{E}^{\tau,k}_\alpha$. We can calculate $\mathcal{E}^{max,k}_\alpha$, and similarly  $\mathcal{E}^{max,k}_\beta$ efficiently with a convex semidefinite program \cite{boyd_vandenberghe_2009}, and return corresponding worst-case covariance matrices $\Sigma_\alpha^{max,k}$ and $\Sigma_\beta^{max,p}$.

% Additionally, we retrieve the covariance matrix $\Sigma^{k,p}$ between poses $\textbf{x}^k_\alpha\in\mathcal{X}_\alpha$ and $\textbf{x}^p_\beta\in\mathcal{X}_\beta$ from the MLE.

% The transformation between pose $\textbf{x}^{t_1}_\alpha\in\mathcal{X}_\alpha$ and $\textbf{x}^{t_2}_\beta\in\mathcal{X}_\beta$ can be achieved by the following smaller transformations
% \begin{align}
%     \textbf{x}^{t_1,t_2}_{\alpha,\beta} = \textbf{x}^{t_2,p}_\beta \oplus \textbf{x}^{p,k}_{\alpha,\beta} \oplus \textbf{x}^{k,t_1}_\alpha
% \end{align}

% Therefore, worst case uncertainty represented by covariance matrix $\Sigma^{max}$ between any pose-pair $(\textbf{x}_\alpha\in\mathcal{X}_\alpha, \textbf{x}_\beta\in\mathcal{X}_\beta)$ is bounded by the combined uncertainty of $\Sigma_\alpha^{max,k}$, $\Sigma_\beta^{max,p}$ and $\Sigma^{k,p}$: \textit{see paper https://arxiv.org/pdf/1906.07795v1.pdf for how to combine uncertainty matrices}.

% From $\Sigma^{max}$ with largest eigenvalue $\lambda_1$ and corresponding eigenvector $v_1$, we can derive the size of the uncertainty buffer $d_{buffer}$ in Figure \ref{fig:trajectory_overlap_finding} as follows
% \begin{align}
%     d_{buffer,x} &= (\lambda_1 \textbf{v}_1 \cdot \begin{bmatrix}1 \\ 0\end{bmatrix}+c)\chi_\gamma\\
%     d_{buffer,y} &= (\lambda_1 \textbf{v}_1 \cdot \begin{bmatrix}0 \\ 1\end{bmatrix}+c)\chi_\gamma
% \end{align}
% where $\cdot$ denotes the inproduct, $c$ is the variance of the Gaussian mapping $(\textbf{x}_\alpha,\textbf{x}_\beta)_{kp} \to p(u_{kp})$, and $\chi_\gamma$ denotes the confidence level of $d_{buffer}$.




\subsection{Identifying direct path in a multipath propagation setting}
% The communication signal can arrive at the robot via $n$ different propagation paths, which form the set of binary variables $\mathcal{P}=\{P_1, P_2, ...,P_n \}$. Here, $P_i=1$ indicates that path $i$ is the direct path. We capture this multipath propagation phenomena in the AOA measurement by modeling this measurement as a multimodal variable, such that $f(\phi)$ is the marginal distribution of multiple Gaussian distributions.
% \begin{align}
%     f(\phi) &= \sum_i^{|\mathcal{P}|} 
%     f^{\alpha,\beta} (\phi | P_i)p(P_i)
% \end{align}
% Each mode $ f^{\alpha,\beta} (\phi | P_i)$ with $P_i\in\mathcal{P}$ results in a different MLE estimate of the poses $\hat{\mathcal{X}}_i$, where we denote the optimized MLE estimate with a hat. We retrieve the MLE estimates of each mode by replacing $f^{\alpha,\beta}(\phi| \textbf{x}_\alpha, \textbf{x}_\beta)$ in equation \ref{eq:MLE} with the Gaussian distribution $f^{\alpha,\beta}(\phi|P_i, \textbf{x}_\alpha, \textbf{x}_\beta)$. Finally, for each $\hat{\mathcal{X}}_i$, we search for the set of candidate inter-robot loop closures $G_\Sigma^i$ (as previously defined in the Problem Statement).
% \begin{align}
%     G_\Sigma^i = \{... | \hat{\mathcal{X}}_i\}
% \end{align}

% Each of the pose-pairs in candidate set $G_\Sigma^i$ is either a true or false loop-closure. Let us define the binary variable $u_{kp}$ for each pose-pair $(\textbf{x}^i_\alpha, \textbf{x}^i_\beta)_{kp}\in G_\Sigma^i$, such that $u_{kp}=1$ if pose-pair $(\textbf{x}^i_\alpha, \textbf{x}^i_\beta)_{kp}$ is a true loop-closure, and $u_{kp}=0$ otherwise. 
Our algorithm will only find correct inter-robot loop closures if the AOA measurement captures the direct path. However, due to the multipath problem, we have a set $\mathcal{P}$ of which maximally one path is the direct path. In this section we show how to apply Bayes rule to provide the probability of some path $P_i\in\mathcal{P}$ being the direct path. \\

First, for a number of inter-robot loop closures $(\textbf{x}^\alpha_p, \textbf{x}^\beta_k)\in G_i$, we check whether they are a match e.g. by applying ICP, bundle adjustment or PCM. This thus provides us with the information $u_{kp}=U_{kp}$ with $U_{kp}=1$ for a successfull match, and $U_{kp}=0$ if the match is rejected. Given the new information, we can update the probability of $P_i$ being the true direct path with Bayes rule.
\begin{align}
    % f(\phi | \textbf{u}) &= \sum_i^{|\mathcal{P}|} f^{\alpha,\beta} (\phi | P_i) \underbrace{p(P_i|u_{kp})}_{w_i(u_{kp})}\\
    % &=\sum_i^{|\mathcal{P}|} f^{\alpha,\beta} (\phi | P_i)\frac{p(u_{kp}|P_i)p(P_i)}{p(u_{kp})}
    p(P_i|u_{kp}=U_{kp}) = \frac{p(u_{kp}=U_{kp}|P_i)p(P_i)}{p(u_{kp}=U_{kp})}
\end{align}
where $p(u_{kp}=U_{kp}|P_i)$ is computed as in equation \ref{eq:prob_true_LC}, $p(P_i)$ is the prior, and $p(u_{kp})$ is some normalization constant such that $\sum_{P_i\in\mathcal{P}}p(P_i|u_{kp})=1$.\\

% We re-use previously defined relations under each hypothesis that path $P_i$ is the true direct path. Thus, the probability that pose-pair $(\textbf{x}_k^\alpha, \textbf{x}_p^\beta)$ is a true inter-robot loop closure, is given by
% ------------------- Mahalanobis method -------------------\\
% \begin{align}
%     p(u_{kp}| P_i, \textbf{x}_p^{\alpha}, \textbf{x}_k^{\beta} ) &= e^{\ - \frac{1}{2}c\| \textbf{x}_p^{\alpha}-\textbf{x}_k^{\beta} \|_2 },\quad c>0\\
% \end{align}
% We can use the same result from Eq. \ref{eq:prob_true_LC} to obtain $p(u_{kp}|P_i)$ by marginalizing over the positions of the pose-pair. The only difference is that we now have an additional conditional dependency on $P_i$ being the true path.
% \begin{align}
%     p(u_{kp} | P_i) &= \int_{\mathbb{R}^d} p(u_{kp} | P_i, (\textbf{x}^i_{\alpha}, \textbf{x}^i_{\beta})_{kp}) f((\textbf{x}^i_{\alpha}, \textbf{x}^i_{\beta})_{kp}|P_i)dx\\
%     % &= \int_{\mathbb{R}^d} e^{\ - \frac{1}{2}c\| \textbf{x}^i_{\alpha,j}-\textbf{x}^i_{\beta,j} \|_2 -\frac{1}{2}\| \Bar{\textbf{x}}+\textbf{x}^i_{\alpha,j}-\textbf{x}^i_{\beta,j} \|_{\Sigma^{-1}}}dx\\
%     % &= e^{-\frac{1}{2}\Bar{\textbf{x}}\Sigma^{-1}\Bar{\textbf{x}}}\int_{\mathbb{R}^d} e^{\ -\frac{1}{2} \textbf{D}^T (\Sigma^{-1} + cI) \textbf{D} - \Bar{\textbf{x}}^T\Sigma^{-1}\textbf{D}}dx\\
%     % &=\sqrt{\frac{(2\pi)^d}{\det (\Sigma^{-1} +cI)}}e^{-\frac{1}{2}\Bar{\textbf{x}}^T\Sigma^{-1}\Bar{\textbf{x}} + \Bar{\textbf{x}}^T\Sigma^{-1} (\Sigma^{-1} +cI)^{-1}\Sigma^{-1}\Bar{\textbf{x}}}
% \end{align}

% ------------------- Binomial method -------------------\\
% If propagation path $P_i$ truly is the direct path, then we expect a large proportion of the pose-pairs in $G_\Sigma^i$ to be true loop-closures, i.e. a large true positive rate (TP).
% \begin{align}
%     E_{kp}[u_{kp}| P_i=1] = TP
% \end{align}
% Meanwhile, if propagation path $P_i$ is not the direct path, there are likely less loop-closures. Therefore, we can use hypothesis testing to compute the probability of observing $m$ true loop closures in $G_\Sigma^i$, given the poses $\mathcal{X}_i$.
% \begin{align}
%     % H_0:\ &E_{kp}[u_{kp} | P_i=1] = TP\\
%     % H_1:\ &E_{kp}[u_{kp} | P_i=0] < TP
%     H_0:\ &p(u_{kp}=1) = TP\\
%     H_1:\ &p(u_{kp}=1) < TP
% \end{align}
% Variable $u_{kp}$ follows the binomial distribution, such that the probability of having $k_b$ true loop closures in a set of $n_b$ loop closure candidates is given by
% \begin{align}
%     P(u_{kp}=k_b)=\begin{pmatrix}n_b \\k_b \end{pmatrix}TP^{k_b} (1-TP)^{n_b-k_b}
% \end{align}
% Hypothesis $H_0$ is then rejected if $P(u_{kp} \leq k_b|P_i=1) \leq \gamma$. \\
% ---------------------------------------------------------------------\\


% For each MLE solution, we can define for any pair of poses $(\hat{\textbf{x}}_{\alpha,i}^k, \hat{\textbf{x}}_{\beta,i}^p)$, the pdf of the distance between these poses, and the corresponding probability $p( \hat{\textbf{x}}_{\alpha,i}^k - \hat{\textbf{x}}_{\beta,i}^p |\ u=1)$.

% \begin{align}
%     f(\hat{\textbf{x}}_{\alpha,i}^k - \hat{\textbf{x}}_{\beta,i}^p) = c e^{ -\frac{1}{2}\| \hat{\textbf{x}}_{\alpha,i}^k - \hat{\textbf{x}}_{\beta,i}^p \|_\Sigma}
% \end{align}
% Then, the probability that a pair of poses are actually in the same position is
% -----------------------------
% \begin{align}
%     f(\phi|\textbf{x}_\alpha,\textbf{x}_\beta)&= \sum_i^{|\mathcal{P}|} 
%     f^{\alpha,\beta}(\phi | P_i, \textbf{x}_\alpha,\textbf{x}_\beta) \underbrace{p(P_i | \textbf{x}_\alpha,\textbf{x}_\beta)}_{w_i}\\
%     % f^{\alpha,\beta}(\phi,P_i |\textbf{x}_\alpha,\textbf{x}_\beta) \\%\underbrace{p(P_i | \textbf{x}_\alpha,\textbf{x}_\beta)}_{w_i}
%     w_i&= \frac{f(\textbf{x}_\alpha,\textbf{x}_\beta | P_i)p(P_i)}{f(\textbf{x}_\alpha,\textbf{x}_\beta)}\\
%     % w_i f^{\alpha,\beta}(\phi_i | \textbf{x}_\alpha,\textbf{x}_\beta) \\
%     \sum_i w_i &= 1 % Direct path not necessarily in here
% \end{align}
% % Assumption: one of the paths is the direct path.
% Relation between propagation path and pose matches.
% % \begin{align}
% %     f^{\alpha,\beta}(\phi|\textbf{x}_\alpha,\textbf{x}_\beta, u)&=f^{\alpha,\beta}(\phi|\textbf{x}_\alpha,\textbf{x}_\beta)f(\textbf{x}_\alpha,\textbf{x}_\beta|u) 
% % \end{align}
% \begin{align}
%     p(P_i | u=U) &= \int_{\mathbb{R}^d} p(P_i | \textbf{x}_\alpha,\textbf{x}_\beta) f(\textbf{x}_\alpha,\textbf{x}_\beta|u=U)dx\\
%     &=p(P_i)\int_{\mathbb{R}^d} \frac{f(\textbf{x}_\alpha,\textbf{x}_\beta | P_i)}{f(\textbf{x}_\alpha,\textbf{x}_\beta)} f(\textbf{x}_\alpha,\textbf{x}_\beta|u=U)dx\\
%     E_u[p(P_i | u&=U)] = p(U_0)p(P_i | u=U_0) \\ &\qquad+ p(U_1)p(P_i | u=U_1)
% \end{align}

Alternatively, %instead of passively updating the probability that some $P_i\in\mathcal{P}$ is the direct path, 
we can actively plan which pose-pairs would provide the most information to differentiate between direct and indirect paths. For this, we minimize Shannon entropy $J = -\sum_i w_i\log (w_i)$, with $w_i = p(P_i)=E_u[p(P_i|u_{kp})]$.
\begin{align}
    \hat{u}_{kp} &= \arg\min_{u_{kp}\in G_{tot}} J(u_{kp})
\end{align}
We narrow the search-space for $u_{kp}$ to $G_{tot}$, which is the union of all $G_i$. After all, inter-robot loop closures that are not part of any $G_i$ are not likely to contain much information on which set $G_i$ corresponds to the true direct path $P_i=1$.

==> Notes.tex <==
\newpage
Log-likelihood function $\log( f_{comm})$, conditional on the the translation $\textbf{x}$ from $\textbf{x}^\alpha$ to $\textbf{x}^\beta$.
\begin{align*}
    \log (f_{comm}(r,\textbf{u}|\textbf{x})) = \frac{1}{\sigma^2} (r-\|\textbf{x}\|_2)^{2} - \kappa  \frac{\textbf{u}^\top \textbf{x}}{\|\textbf{x}\|_2}
\end{align*}

Linearizing above pdf results in a Gaussian of which covariance matrix $\Sigma$ is computed as [REF: Ranging-Based Localizability-Constrained Deployment of Mobile Robotic Networks]
\begin{align*}
    \Sigma = \left( -E_\textbf{z}\left[ \frac{\partial^2 \log f(\textbf{z}|\textbf{x})}{\partial \textbf{x}^2}\ \bigg| \ \textbf{x} \right] \right)^{-1}
\end{align*}
A useful website for computing the derivate $\frac{\partial^2 \log f}{\partial \textbf{x}^2}$: \\ \textit{matrixcalculus.org}

\begin{align*}
    H =& \frac{\partial^2 \log f}{\partial \textbf{x}^2} = \frac{\partial^2}{\partial \textbf{x}^2} \left( \frac{1}{\sigma^2} (r-\|\textbf{x}\|_2)^{2} - \kappa  \frac{\textbf{u}^\top \textbf{x}}{\|\textbf{x}\|_2}\right) \\[4pt]
    =& \frac{\partial}{\partial \textbf{x}} \left( \frac{2 (r-\|\textbf{x}\|_2)}{\sigma^2 \|\textbf{x}\|_2 } \textbf{x} -\frac{\kappa}{\|\textbf{x}\|_2} \textbf{u} + \frac{\kappa\ \textbf{x}^\top \textbf{u}}{\|\textbf{x}\|_2^{3}} \textbf{x} \right)\\[4pt]
    =& - \frac{(3 \kappa\ \textbf{x}^\top \textbf{u})}{\|\textbf{x}\|_2^{5}} \textbf{x} \textbf{x}^\top + \frac{\kappa}{\|\textbf{x}\|_2^{3}}\textbf{u} \textbf{x}^\top + \frac{\kappa}{\|\textbf{x}\|_2^{3}}\ \textbf{x} \textbf{u}^\top + \frac{\kappa\ \textbf{x}^\top \textbf{u}}{\|\textbf{x}\|_2^{3}} \mathbb{I}  \\
    & - \frac{2 (r-\|\textbf{x}\|_2)}{\sigma^2 \|\textbf{x}\|_2^{3}} \textbf{x} \textbf{x}^\top  
     - \frac{2}{\sigma^2 \|\textbf{x}\|_2^{2}}\ \textbf{x} \textbf{x}^\top + \frac{2 (r-\|\textbf{x}\|_2)}{\sigma^2\|\textbf{x}\|_2} \mathbb{I}\\[8pt]
    H_{ij} =& -  \frac{3 \kappa}{\|\textbf{x}\|_2^{5}} \sum_k x_i x_j x_k u_k  + \frac{\kappa}{\|\textbf{x}\|_2^{3}}  \sum_l x_l \delta_{ij} u_l  \\ &+ \frac{\kappa}{\|\textbf{x}\|_2^{3}}x_j u_i + \frac{\kappa}{\|\textbf{x}\|_2^{3}}\ x_i u_j  \\
    & + \left(\frac{2}{\sigma^2 \|\textbf{x}\|_2^{3}}x_i x_j + \frac{2}{\sigma^2\|\textbf{x}\|_2} \delta_{ij} \right) r \\
    & + \frac{2}{\sigma^2 \|\textbf{x}\|_2^{2}} x_i x_j - \frac{2\|\textbf{x}\|_2}{\sigma^2 \|\textbf{x}\|_2^{3}}x_i x_j - \frac{2 \|\textbf{x}\|_2}{\sigma^2\|\textbf{x}\|_2} \delta_{ij} \\[8pt]
    E_\textbf{z}[H_{ij} | \textbf{x}] =& -  \frac{3 \kappa}{\|\textbf{x}\|_2^{5}} \sum_k x_i x_j x_k E[u_k]  + \frac{\kappa}{\|\textbf{x}\|_2^{3}}  \sum_l x_l \delta_{ij} E[u_l]  \\ &+ \frac{\kappa}{\|\textbf{x}\|_2^{3}}x_j E[u_i] + \frac{\kappa}{\|\textbf{x}\|_2^{3}}\ x_i E[u_j]  \\
    & + \left(\frac{2}{\sigma^2 \|\textbf{x}\|_2^{3}}x_i x_j + \frac{2}{\sigma^2\|\textbf{x}\|_2} \delta_{ij} \right) E[r] \\
    & + \frac{2}{\sigma^2 \|\textbf{x}\|_2^{2}} x_i x_j - \frac{2\|\textbf{x}\|_2}{\sigma^2 \|\textbf{x}\|_2^{3}}x_i x_j - \frac{2 \|\textbf{x}\|_2}{\sigma^2\|\textbf{x}\|_2} \delta_{ij} \\[10pt]
    E[u_0] =& E[sin(b\alpha)] = e^{-\frac{1}{2}\sigma^2b^2}\sin (\mu b), \quad \alpha \sim \mathcal{N}(\mu, \sigma) \\
    E[u_1] =& E[cos(b\alpha)] = e^{-\frac{1}{2}\sigma^2b^2}\cos(\mu b) 
%\int_{-\infty}^\infty \int_{-\infty}^\infty H_{ij} f_\textbf{U}(\textbf{u)} f_R (r) d\textbf{u} dr
\end{align*}
